Differentially Private Heavy Hitter Detection using Federated Analytics

In this work, we study practical heuristics to improve the performance of prefix-tree based algorithms for differentially private heavy hitter detection. Our model assumes each user has multiple data points and the goal is to learn as many of the most frequent data points as possible across all users' data with aggregate and local differential privacy. We propose an adaptive hyperparameter tuning algorithm that improves the performance of the algorithm while satisfying computational, communication and privacy constraints. We explore the impact of different data-selection schemes as well as the impact of introducing deny lists during multiple runs of the algorithm. We test these improvements using extensive experimentation on the Reddit dataset~\cite{caldas2018leaf} on the task of learning the most frequent words.

==> A03a-Algorithms.tex <==
\section{Further Algorithm Details and Pseudo-code}\label{sec:alg-details}












==> Outline.tex <==
\begin{itemize}


    \item Importance of federated statistics for unknown dictionary
    \begin{itemize} 
    \item different data selection schemes
    \item starting from single data point per user
    \item multiple data points per user, draw randomly
    \item multiple data points per user, considering the prefix lst for selecting the datapoint
    \item multiple data points per user, considering the prefix lst and deny list for selecting the datapoint
    \end{itemize}
    \item Hyper Parameter tuning effect on the utility 
    \begin{itemize}
        \item Segment length (Uniform, Non-Uniform)
        \item Number of iterations
    \item Confidence per iteration (Dynamically set based on the False Positive ratio)
    \item Decompression Constraints
    \item (not sure) Privacy management (uniform Vs Non-uniform)
    \item Sampling

    \end{itemize}
    \item comparison with Google paper~\cite{zhu2020federated} and non-interactive version. 
    \item evaluation datasets are Reddit and Twitter dataset~\cite{go2009twitter}. 
\end{itemize}
